A unifying framework for generalised Bayesian online learning in non-stationary environments

We propose a unifying framework for methods that perform probabilistic online learning in non-stationary environments. We call the framework BONE, which stands for generalised (B)ayesian (O)nline learning in (N)on-stationary (E)nvironments. BONE provides a common structure to tackle a variety of problems, including online continual learning, prequential forecasting, and contextual bandits. The framework requires specifying three modelling choices: (i) a model for measurements (e.g., a neural network), (ii) an auxiliary process to model non-stationarity (e.g., the time since the last changepoint), and (iii) a conditional prior over model parameters (e.g., a multivariate Gaussian). The framework also requires two algorithmic choices, which we use to carry out approximate inference under this framework: (i) an algorithm to estimate beliefs (posterior distribution) about the model parameters given the auxiliary variable, and (ii) an algorithm to estimate beliefs about the auxiliary variable. We show how the modularity of our framework allows for many existing methods to be reinterpreted as instances of BONE, and it allows us to propose new methods. We compare experimentally existing methods with our proposed new method on several datasets, providing insights into the situations that make each method more suitable for a specific task. We provide a Jax open source library to facilitate the adoption of this framework.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/MAP-weights.tex <==
\section{Weights as MAP Estimates}



\subsection{Weighted Dynamics}

We now introduce a scale mixture model on the dynamics step
\begin{equation}
p\left(\vtheta_{t}\vert\vtheta_{t-1}\right)=\gauss\left(\vtheta_{t}\vert\vtheta_{t-1},v_{t}^{-1}\vQ_{t}\right)
\end{equation}
Assuming a Gamma prior on $v_{t}$ yields the model
\begin{align}
p\left(\vy_{t}\vert\vx_{t},\vtheta_{t},w_{t}\right) & =\gauss\left(\vy_{t}\vert\bar{h}_{t}\left(\vtheta_{t}\right),w_{t}^{-1}\vR_{t}\right)\\
p\left(\vtheta_{t}\vert v_{t},\data_{1:t-1}\right) & =\gauss\left(\vtheta_{t}\vert\vmu_{t-1},\vSigma_{t-1}+v_{t}^{-1}\vQ_{t}\right)\\
p\left(w_{t}\right) & ={\rm Gamma}\left(\alpha,\beta\right)\\
p\left(v_{t}\right) & ={\rm Gamma}\left(\gamma,\delta\right)
\end{align}
This model has an important symmetry between inference for $v_{t}$
and $w_{t}$:
\begin{align}
p\left(\vy_{t}\vert\vx_{t},v_{t},w_{t},\data_{1:t-1}\right) & =\int p\left(\vy_{t}\vert\vx_{t},\vtheta_{t},w_{t}\right)p\left(\vtheta_{t}\vert v_{t},\data_{1:t-1}\right){\rm d}\vtheta_{t}\\
 & =\gauss\left(\vy_{t}\vert\hat{\vy}_{t},\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+v_{t}^{-1}\vH_{t}\vQ_{t}\vH_{t}^{\top}+w_{t}^{-1}\vR_{t}\right)\label{eq:yt-given-vt-wt}
\end{align}
That is, $v_{t}^{-1}\vH_{t}\vQ_{t}\vH_{t}^{\top}$ and $w_{t}^{-1}\vR_{t}$
play identical roles in the likelihood once we integrate out $\vtheta_{t}$.
This suggests that whatever weighting function we use, it should be
the same for $V_{t}$ with respect to $\vH_{t}\vQ_{t}\vH_{t}^{\top}$
as it is for $W_{t}$ with respect to $\vR_{t}$.
\begin{align}
W_{t} & =f\left(\ve_{t},\vR_{t}\right)\\
V_{t} & =f\left(\ve_{t},\vH_{t}\vQ_{t}\vH_{t}^{\top}\right)
\end{align}

Paralleling Section (\ref{subsec:Prior-Uncertainty}) the joint posterior
on $v_{t},w_{t}$ is 
\begin{align}
p\left(v_{t},w_{t}\vert\data_{1:t}\right) & \propto p\left(v_{t}\right)p\left(w_{t}\right)p\left(\vy_{t}\vert\vx_{t},v_{t},w_{t},\data_{1:t-1}\right)\\
 & \propto v_{t}^{\gamma-1}w_{t}^{\alpha-1}\left|\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+v_{t}^{-1}\vH_{t}\vQ_{t}\vH_{t}^{\top}+w_{t}^{-1}\vR_{t}\right|^{-1/2}\nonumber\\
 &\qquad\times\exp\left(-\delta v_{t}-\beta w_{t}-\frac{1}{2}\ve_{t}^{\top}\left(\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+v_{t}^{-1}\vH_{t}\vQ_{t}\vH_{t}^{\top}+w_{t}^{-1}\vR_{t}\right)^{-1}\ve_{t}\right)\label{eq:vt-wt-marginal}
\end{align}
As with (\ref{eq:wt-marginal}) there does not seem to be a closed
form maximum for $v_{t}$ or $w_{t}$. If we ignore prior variance
and observation noise ($\vSigma_{t-1}=\vR_{t}=\bm{0}$) for estimating
$v_{t}$ and ignore prior variance and dynamics ($\vSigma_{t-1}=\vQ_{t}=\bm{0}$)
for estimating $w_{t}$ then we get
\begin{align}
v_{t}^{*} & =\frac{\gamma-1+\frac{n_{y}}{2}}{\delta+\frac{1}{2}\ve_{t}^{\top}\left(\vH_{t}\vQ_{t}\vH_{t}^{\top}\right)^{-1}\ve_{t}}\\
w_{t}^{*} & =\frac{\alpha-1+\frac{n_{y}}{2}}{\beta+\frac{1}{2}\ve_{t}^{\top}\vR_{t}^{-1}\ve_{t}}
\end{align}
Therefore if we set the hyperparameters as
\begin{align}
\alpha & =\gamma=\frac{c^{2}-n_{y}+2}{2}\\
\beta & =\delta=\frac{c^{2}}{2}
\end{align}
then the weights become
\begin{align}
V_{t} & =\sqrt{v_{t}^{*}}=\left(1+\frac{\left\Vert \ve_{t}\right\Vert _{\left(\vH_{t}\vQ_{t}\vH_{t}^{\top}\right)^{-1}}^{2}}{c^{2}}\right)^{-1/2}\\
W_{t} & =\sqrt{w_{t}^{*}}=\left(1+\frac{\left\Vert \ve_{t}\right\Vert _{\vR_{t}^{-1}}^{2}}{c^{2}}\right)^{-1/2}
\end{align}

As an alternative to ignoring the variance components that do not
scale with $v_{t}$ or $w_{t}$, we could treat them as though they
do scale. Thus for approximating $v_{t}^{*}$ we would approximate
(\ref{eq:yt-given-vt-wt}) as
\begin{align}
p\left(\vy_{t}\vert\vx_{t},v_{t},w_{t},\data_{1:t-1}\right) & \approx\gauss\left(\vy_{t}\vert\hat{\vy}_{t},\underline{v_{t}^{-1}}\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+v_{t}^{-1}\vH_{t}\vQ_{t}\vH_{t}^{\top}+\underline{v_{t}^{-1}}\vR_{t}\right)
\end{align}
and similarly for approximating $w_{t}^{*}$. This leads to
\begin{align}
V_{t}=W_{t} & =\left(1+\frac{\left\Vert \ve_{t}\right\Vert _{\left(\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+\vH_{t}\vQ_{t}\vH_{t}^{\top}+\vR_{t}\right)^{-1}}^{2}}{c^{2}}\right)^{-1/2}
\end{align}
This seems reasonable from a robust GB perspective because it directly compares the prediction error $\ve_t$ to the predictive variance $\vH_{t}\vSigma_{t-1}\vH_{t}^{\top}+\vH_{t}\vQ_{t}\vH_{t}^{\top}+\vR_{t}$.

==> sections/analysis.tex <==
\section{Algorithmic Analysis}
In the previous section, we demonstrated that the BONE framework recovers many existing methods from the literature.
A natural question that follows is how to select the most appropriate method among them.

In this section, we show how the BONE framework provides new insights into both novel and existing methods.
Specifically, we offer a mathematical analysis demonstrating that for certain
algorithms expressed as BONE components, although operating differently, produce identical predictions for $\vy_{t+1}$.
This highlights the equivalence in prediction under different assumptions of non-stationarity.

Additionally, we show that for some methods proposed as benchmark to novel methods,
involve different choices of BONE components
This raises the question of which components contribute most significantly to improving model performance.
We focus particularly on two claims:
the first from \cite{li2021onlinelearning}, which asserts that the Variational Beam Search algorithm outperforms the BOCD algorithm from \cite{adams2007bocd};
and the second from \cite{titsias2023kalman}, which suggests that the adaptive variant of the EKF method performs better than the traditional EKF.

To the best of our knowledge, this is the first study that examines the equivalence among methods under this perspective.

\subsection{Equivalence among methods}
In this Section, we show that a unique choice of BONE components do not determine a unique estimation for $\hat{\vy}_t$.

\begin{proposition}
    Consider a dataset $\data_{1:t}$ where $\data_t = (\vy_t,)$ and $\vx_t = \emptyset$,
    modelled a multivariate Gaussian with known covariance matrix $\vLambda$, i.e.,
    $p(\vy_t \cond \vtheta) = {\cal N}(\vy_t \cond \vtheta, \vLambda)$,
    Consider, $h(\vtheta, \vx) = \vtheta$ and
    assume a Gaussian conditional prior of the form \eqref{eq:conditional-prior-gaussian}.
    Now, consider the following two configurations of BONE:

    \underline{Configuration 1}:
    Let \texttt{CPL} be the auxiliary variable, so that $\auxv_t = s_{1:t}$.
    Take $\tau_t$ to be of the form \eqref{eq:conditional-prior-gaussian},
    with functions $g$ and $G$ defined as 
    \begin{equation}
    \begin{aligned}
        g(s_{1:t}, \data_{1:t-1}) &= s_t\,\vmu_0 + (1 - s_t)\,\vmu_{(s_{1:t-1})}, \\
        G(s_{1:t}, \data_{1:t-1}) &= s_t\,\vSigma_0 + (1 - s_t)\,\vSigma_{(s_{1:t-1})}.
    \end{aligned}
    \end{equation}
    Finally, let the weighting function $\nu_t$ be of the form \eqref{eq:weighting-marginal-posterior},
    with transition dynamics $p(s_{1:t} \cond s_{1:t-1})$ of the form \eqref{eq:transition-cpl-independent}.

    \underline{Configuration 2}:
    Let \texttt{RL} be the auxiliary variable, so that $\auxv_t = r_t$.
    Take $\tau_t$ be be of the form \eqref{eq:conditional-prior-gaussian}
    with $g$ and $G$ of the form \eqref{eq:gauss-conditional-prior-rl-lookback}.
    Finally, let the weighting function $\nu_t$ be of the form \eqref{eq:weighting-marginal-posterior}
    with transition dynamics $p(r_t \cond r_{t-1})$ of the form \eqref{eq:transition-rl-markov}.

    Then, using \texttt{Conj} updates as $\lambda_t$,
    both Configuration 1 and Configuration 2 yield equivalent predictions for $\vy_{t+1}$, given $\data_{1:t}$.
\end{proposition}
\begin{proof}
    \gdm{
        First show that both conditional posteriors are the same.
        As a consequence, we have the the posterior predictive is the same.
        Finally, we show that all of the weights are the same.
    }
\end{proof}

\begin{proposition}
    \gdm{For the case above, using the multiplicative covariance inflation yields the same result.}
\end{proposition}

\subsection{Worked examples}\label{sec:the-new-methods}
\gdm{Decomponse varitional Beam search into its component and analyse claims over BOCD}
\gdm{Decomponse O-EKF into its component and analyse claims over EKF}

\subsection{How to choose a combination??}
\gdm{Some theoretical analysis before diving into the experiments?}

While the \CACI has been considered in the past,
recent works have argued that adaptivity in Kalman filtering can only be achieved if the dynamics are learned \cite{titsias2023kalman}.
However, we find that a well-tuned constant covariance inflation performs comparable to previously-proposed methods;
see Figure \ref{fig:kf-with-fixed-dynamics} in the appendix.

==> sections/literature-review.tex <==
\section{Worked examples}
\label{sec:related}
In this section, we provide to detailed use-cases of our framework
using modelling choices \cModel, \cAux, \cPrior and algorithmic choices \cPosterior and \cWeight.

First, we derive the classical BOCD algorithm of \cite{adams2007bocd} for a linear Gaussian model.
Next, we derive the mixture of experts' method of \cite{chaer1997mixturekf}.
Finally, we derive a novel method, which we call SPR.

This gives light on the flexibility of our method to accomodate multiple methods.

\subsection{The BOCD method}


% The literature on adaptation to non-stationarity is vast and touches on the fields
% of game-theory, online-convex optimisation, Bayesian filtering, changepoint detection and segmentation,
% among others.

% Changepoint detection (or segmentation) methods have a long-standing history
% in the signal processing literature \cite{basseville1993onlinedetection}.
% Their main goal is the detection of changepoints, rather than the parametric adaptation that occurs in an online learning setting
% \cite{van2020evaluation}.
% In non-Bayesian methods, the problem of online learning in non-stationary environments
% is called concept drift; see \cite{gama2014surveyadaptive, lu2018conceptdrift} for a survey.
% Alternative non-Bayesian OCL methods include \cite{diethe2019ocl, dohare2024continualbackprop}.

% A number of Bayesian approaches that tackle the OCL problem rely on so-called
% replay-buffers.
% These methods allow the algorithm to  update continually and tune model parameters based on previously-seen data points
% \cite{nguyen2017vcl, kurle2019continual, nassar2022bam, beronov2021replaysmc, Kessler2023bayescl}.

% In the filtering literature, various methods have been proposed to adapt to non-stationarity in
% time-series datasets. These methods usually model the covariance structure of the dynamics of the state-space model \cite{mehra1972adptivefiltering, huang2020slide, vilmarest2021viking}.
% %However, they are not easy to write as choices of \cAux, \cPrior, and \cPosterior.



% Non-stationarity has also been studied in other areas of machine learning such as reinforcement learning.
% For instance, the work in \cite{nikishin2023deeprl}
% attributes the under-performance of reinforcement learning methods to either loss of plasticity or the inability to explore.



% GERARDO LEE ESTO:
% Furthermore, the work in \cite{asadi2024rlreset, asadi2024tdoptimisation}
% show that popular deep reinforcement learning algorithms solve a sequence of optimisation problems, where the target loss function change per iteration.
 
